Instructed to Bias: Instruction-Tuned Language Models Exhibit Emergent Cognitive Bias

Recent studies show that instruction tuning (IT) and reinforcement learning from human feedback (RLHF) improve the abilities of large language models (LMs) dramatically. While these tuning methods can help align models with human objectives and generate high-quality text, not much is known about their potential adverse effects. In this work, we investigate the effect of IT and RLHF on decision making and reasoning in LMs, focusing on three cognitive biases - the decoy effect, the certainty effect, and the belief bias - all of which are known to influence human decision-making and reasoning. Our findings highlight the presence of these biases in various models from the GPT-3, Mistral, and T5 families. Notably, we find a stronger presence of biases in models that have undergone instruction tuning, such as Flan-T5, Mistral-Instruct, GPT3.5, and GPT4. Our work constitutes a step toward comprehending cognitive biases in instruction-tuned LMs, which is crucial for the development of more reliable and unbiased language models.

==> Sections/04_cog_biases_old.tex <==
\section{Cognitive Biases}\label{sec:cog_biases}
We propose to investigate the extent to which different language models display cognitive-like biases similar to those observed in human behavior.

A cognitive bias refers to systematic patterns of deviation from rational or logical thinking, leading individuals to make judgments or decisions that are influenced by subjective factors, preconceptions, or inherent cognitive limitations rather than objective evidence or rationality.
Cognitive-like biases can be measured by a shift in preferences or choices triggered by contextual or alternative changes, which, from a rational or logical perspective, should not have a significant impact.

% Given the diverse range of cognitive biases, we have chosen to focus on three well-established biases: the \textit{Decoy Effect}, \textit{Certainty Effect}, and \textit{Belief Bias}.

Our investigation centered on the decoy effect, certainty effect, and belief bias, which are distinctive biases associated with decision-making and judgment.
The decoy and certainty effects specifically address various facets of prospect theory and possess notable characteristics that enhance their distinctiveness.
The belief bias represents a judgment-related bias and has previously been observed in a different pretrained model, making it an interesting additional bias to explore.

% \nir{perhaps write some more on cognitive biases in general, and ours in particular? give some history, context, describe their scope and prevalence, etc}
% \itay{I suspect it would be too much for the average NLP reader. We can refer to a survey maybe?}

\subsection{Decoy Effect}
When making comparative judgments of value, individuals often assess multiple options based on various choice criteria.
A decoy option strategically serves as a reference point to another option by intentionally appearing inferior, thereby influencing the perception of the other option as dominant and preferable.

The decoy effect materializes when humans are presented with two options, and will tend to have a specific change in preference when also presented with a third decoy option that is asymmetrically dominated \cite{Huber1981AddingAD}.
An option is asymmetrically dominated (\textit{Decoy Option}) when it has a lower rating in all dimensions compared to one option (\textit{Target Option}); but, in comparison to the other option, it has a lower rating in some dimensions and higher in others (\textit{Competitor Option}).

Given pre-chosen Target and competitor options with two-dimensional quality ratings, the definition for a decoy option gives us a specific range of possible values that a third option within these values range will be considered a decoy.

\subsection{Certainty Effect}
In situations where choices involve uncertain outcomes,  Individuals generally prefer options with a higher expected value, taking into account the probability of each outcome. 
However, this preference may shift when one option is presented as \textit{certain}, leading to a preference for options with lower expected value but greater certainty.
% tend to display a preference for options with guaranteed or certain outcomes, even when the expected value of an alternative option is objectively higher.
The certainty effect describes the phenomenon where people underweight outcomes that are merely probable in comparison with outcomes that are obtained with \textit{certainty} as shown by \cite{Kahneman1979ProspectTA}.

In the same work \citet{Kahneman1979ProspectTA} show another adjacent effect where people underweight probabilities of outcomes that are possible but not probable (e.g. probabilities lower than 0.03), but overweight probabilities when they are merely probable.
We aggregate these effects together, as the source of bias is the same and results trend are similar.
%That is,  individuals prefer options with a higher expected value, taking into account the probability of each outcome.
%However, this preference may shift when one option is presented as \textit{certain}, leading to a preference for options with lower expected value but greater certainty.

\subsection{Belief Bias}
Syllogisms are a class of reasoning problems characterized by a straightforward argument structure, involving two true statements that logically necessitate a third statement \cite{smith2000aristotle}. 
These multi-step reasoning tasks provide an essential framework for investigating deductive reasoning abilities and the cognitive processes involved in drawing valid conclusions.

Belief bias occurs when a person evaluates the strength of an argument based on their beliefs about the world and personal values, rather than actual evidence presented with the two true statements in the argument.

This bias was shown in a series of experiments where human subjects were given sets of two premises and a conclusion and asked whatever the conclusion followed directly from the premises \cite{evans1983conflict}.
Half of the conclusions were created so they would be \textit{believable} - aligned with general world knowledge (e.g., "cigarettes are addictive"), and the other half was constructed to be \textit{Unbelievable} ("cigarettes are non-addictive").

The results showed that humans were more likely to consider believable conclusions as valid and unbelievable conclusions as invalid, highlighting the presence of belief bias.

In recent work, \citet{dasgupta2022language} showed that the Belief bias exists in Chinchilla  \citep{hoffmann2022training}.
Our work recreates their results on this bias and expands them to other models.




==> Sections/05_data_gen.tex <==


\section{Data Generation}
\label{sec:appendix_data_generation}
% \gabis{Also, I think we should have a central place for examples of the different biases, e.g., in a nice table which can act as reference for readers throughout the paper. Then the text here can interact with the table: ``For the decoy bias, we see in Table ...''}

% \gabis{I think the text here abuses the verb ``create'' here. Maybe before starting to describe each bias, describe this ``creation'' process? Are there any common elements in writing the examples to all biases? }
% \itay{I rephrased every 'create' in here to a more suitable word in each case (not sure if that is what you meant).
% I also added a common element, but most of the description is specific for each bias.}

\input{Sections/Tables/data_numbers}

To thoroughly examine the models and mitigate potential confounders we carefully design a range of prompts to assess the models' susceptibility to the three biases.
We generate an extensive collection of \biaseddataset{} and control samples, encompassing various options' values, textual templates, and permutations of option order.

By employing this approach, we aim to introduce substantial variability among the samples while ensuring independence from the original papers' examples, thus minimizing the risk of data contamination.
We elaborate on the data generation process of each one of the biases.
A table representing the total number of samples in each bias is in Table \ref{appendix:tab:data_numbers}


\subsection{Decoy Effect Data}
\label{subsec:data_gen_decoy}
To generate the data for the decoy effect, we follow \cite{huber1982adding} and compose a set of textual prompts, each posing a selection from four different product categories: cars, phones, frying pans, and real estate properties.
Depending if the sample is from the control or from the \biaseddataset{} dataset, each example involved either two or three product alternatives, each with two attributes - product price and quality rating.

In each conditions, we compared two conditions:
% \nir{`setting' sounds like something you make comparisions within -- not accross.}
% \nir{as i said, i would save the word `bias' for the general effect and measurement; consider calling this `control' and `treatment' instead}
\begin{enumerate}
    \item \textbf{Control -- Two Options} Two options are presented: the \textit{Target Option} and the \textit{Competitor Option}.
    \item \textbf{\Biaseddataset{} -- Third Decoy Option} Three options are presented. In addition to \textit{Target Option} and \textit{Competitor Option}, we added the \textit{Decoy Option}.
    % \item \textbf{False Decoy} Three options are presented. \textit{Target Option} and \textit{Competitor Option},  and we add a third \textit{Decoy Option} which is deliberately chosen \textit{not} to be a decoy option according to the definition to act as a control.
\end{enumerate}

We chose price values according to the actual price ranges from web consumer stores or by prompting the model for a reasonable price range.
We chose low-end and high-end products as our two options in the control condition.

To create the decoy option, we follow \citep{huber1982adding} and create four possible decoys according to the target option, each is worse than the target in the price dimension (more expensive, same quality), or the quality dimension (less quality, same price), or a combination of both.


We constructed variations with different price and quality gaps between the options, five different textual templates, and permutations between the location of each option.


\subsection{Certainty Effect Data}
Similarly to the decoy effect, we follow the original work by \citet{kahneman1979prospect} to generate our data.
In both conditions,  two options for getting prize money with different probabilities are presented. One option is with a lower excepted utility than the other (\textit{Target}) while the other option with a higher excepted utility (\textit{Higher Excepted Value}).

% \nir{could we rewrite this to emphasize that both conditions are the same expect that in the treatment condition `high probability' is actually 1?}
\begin{enumerate}
\item \textbf{\Biaseddataset{} - Certainty} The lower excepted utility \textit{Target} option is certain, while the other option with a higher excepted utility is given at some probability (\textit{Higher Excepted Value}).
\item \textbf{Control - No Certainty} The lower excepted utility \textit{Target} option has a higher probability, while the other option (\textit{Higher Excepted Value})  has a higher excepted utility with a lower probability.
\end{enumerate}

In both conditions, the probability gap between the options was held constant.
For instance, in the \biaseddataset{} condition, if one option was certain (100\%) and the other option had an 80\% chance of yielding a reward, the corresponding options in the control condition would have a 20\% probability gap.
% We obtained the values for prize rewards and probabilities from \cite{Kahneman1979ProspectTA} and also included additional values that maintained the same relationships.
% \nir{i would start the paragraph with this; otherwise readers will think we've invented this experimental paradigm (and only then find out we didn't)}

Similar to the decoy effect, we used a diverse set of prompts using 4 different sub-template combinations and options permutations to create our test set.

\input{Sections/Tables/table_not_probable}

\subsection{Belief Bias Data}

To explore the belief bias in LMs we conduct our experiments using the data generated by \citet{dasgupta2022language}.

% To explore the Belief bias in LMs we also conduct two experiments.
The model is presented with two premises and a conclusion and instructed to choose if the conclusion stems directly from the premises.
If the conclusion logically stems from the premises the model should output 'Valid', otherwise, it should output 'Invalid'.

Here there are two conditions, the bias condition where each argument is believable or unbelievable, and the control condition where the arguments are neutral in terms of believability.
% To control the effect of believability on the performance of the model we run a control experiment, in which we use a different set of objects in each experiment.
% \nir{not really clear what the treatment is at this point}

\begin{enumerate}
    \item \textbf{\Biaseddataset{} - Real-Life Objects } The objects the logical reasoning is based on \textit{real-life} objects, which can have believable or unbelievable nature according to world knowledge (e.g. ``cigarettes are addictive'' as believable, ``cigarettes are non-addictive'' as unbelievable).
    .\item \textbf{Control - Non-real Objects}  The objects the logical reasoning is based on our \textit{non-real} objects using made-up words, which do not have believable or unbelievable nature according to world knowledge (e.g ``wobars are shnesive'' and ``wobars are non-shnesive''), which create neutral arguments.
\end{enumerate}

The valid-believable and invalid-unbelievable conclusions in the condition of the Real-life object are considered as consistent conclusions and valid-unbelievable and invalid-believable are the inconsistent conclusions.
% In this bias, since there is a correct answer we can also measure the model accuracy on the task.
See \citet{dasgupta2022language} for more details on the belief bias data generation process.

% The real-life objects were taken from the original work on Belief bias \cite{evans1983conflict}.
% The non-real objects were created with made-up words that follow the grammatical English rules.

% To generate the non-real samples, we transformed each real-life sample by replacing each real-life object with a corresponding non-real object ("cigarettes" $\rightarrow$ "wobars"; "addictive" $ \rightarrow $ "shnesive").
% % This resulted in a set of non-real samples that were split into believable and unbelievable groups based on their alignment with real-life samples, even though believability has no meaning in the context of non-real objects.
% % This split allows for easier comparison of the results with those of real-life objects.

% We designed the data such that each conclusion could be either valid or invalid and believable or unbelievable, and we included an equal number of samples for each combination of attributes. To create a diverse set of samples, we used 5 different text templates and 3 different object sets, resulting in a total of 766 samples after permuting the premises.

% Beyond using our own data, we also used data from \cite{dasgupta2022language} where they used hand-crafted real-life objects which allow a higher level of unbelievability, and we report our result for both datasets.


==> Sections/07_evaluation.tex <==
%\subsection{Evaluation}
%\label{sec:eval}
% \gabis{Better not to leave the preamble for sections (e.g., here 5.0) empty. Instead use this space to link what we've seen previously with what we'll see next. Give a TOC description of the subsections, e.g., ``In Section 5.1 we will discuss, finding that ... Then in Section 5.2 ..., Finally in Section 5.3...'' This again allows readers to skim (which is good!)}

% In each of the conducted experiments, an assessment is performed on the model outputs to gauge the level of bias exhibited by the model.
% The extraction of the model answer from its output is detailed in Section \ref{subsec:eval_ans}.
% The definition and interpretation of bias scores are expounded upon in Section \ref{subsec:bias_score}, elucidating the metrics used to quantify biases.
% Furthermore, Section \ref{subsec:few_shot} outlines an additional setting implemented in the experiments, namely the few-shot setting, which merits further discussion and analysis.


\subsection{Determining the Model's Answer}
\label{subsec:eval_ans}
% \gabis{On the whole on the one hand this seems like a small implementation issue, otoh, I couldn't understand what we're actually doing. So we don't do this for the instruction-tuned models? only for the non-instruction?}
Given a prompt asking for a choice, the instruction-tuned models usually generate text describing their choice, simply as generating ``Option 1'' or ``Brand 2''.\footnote{In the certainty effect less than \%5 of the predictions made by Flan-T5-XXL were not clear and we excluded these example}

To assess the pretrained performance for each task, we use the common practice \cite{brown2020language} of evaluating the likelihood of various candidate answers from a predefined set of possible answers. 
This evaluation might be affected by a preference of the model to an answer given the context (e.g. given ``Answer:'' the model might give a higher baseline probability to ``Option 2'').
We apply the DC-PMI correction \cite{holtzman-etal-2021-surface} that mitigates this issue by normalizing each answer likelihood within the context of the prompt, relative to a baseline prompt (``Answer:'' in our case).

% \gabis{worth mentioning that this is a common approach (e.g., Maarten Sap does this in his TOM papers)}
% These answers are evaluated independently, with the model not being exposed to all answer choices simultaneously during the selection process. \gabis{I don't understand this last part about independent evaluation}

% This evaluation might be affected by a preference of the model to an answer given the context (e.g. given "Answer:" gives a higher probability to "Option 2").
% To mitigate this potential issue, \citet{holtzman-etal-2021-surface} suggested the DC-PMI correction. 
% % \gabis{This statement presupposes that the reader knows what is this issue. Instead rephrase to say: ``It was observed that models suffer from ... since .... To mitigate this Holtmzan et al proposed...''}
% This correction involves measuring the change in the likelihood of each answer within the context of the question, relative to a baseline context ("Answer:" in our case).
% Consequently, the answer with the highest increase in likelihood within the given context is selected.

% In some cases, the normalization did not change the model preferences, but in others, we noticed the normalization had a strong effect that does not necessarily represent the model preference best.
% For example, in the Belief bias data set we can measure the accuracy of the model as
% In our experiments results we report both normalized and unnormalized scores.

\input{Sections/Tables/gpt4_results}

\subsection{Using Few-shot}
\label{subsec:few_shot}
% The decoy effect and certainty datasets used in our study are characterized by their choice-dependent nature, as they are decision-making biases wherein a clear and unequivocal correct answer does not exist.
% Consequently, the zero-shot setting aligns most effectively with our objective of assessing the model's bias with minimal external influence.
The decoy and certainty effects samples are choice-dependent questions with no ``correct'' answer.
Recent work suggested that giving few-shot samples without the correct labels could improve model performance by introducing the model with the overall format of
the samples \cite{min2022rethinking}.
% In our case, giving as examples samples with random answers could still affect the model since each answer is either biased or unbiased and could teach the model that this is the desired behavior and comprise the results.
Inspired by this work, instead of providing few-shot samples with correct labels, we explore a variation called ``format few-shot'' that omits the original \biaseddataset or control samples.
This approach aims to familiarize the model with the sample format without biasing it in any particular direction.

In the format few-shot approach, we manually curate examples for the decoy and certainty effects, presenting choices between arbitrary options (e.g., ``Which would you prefer, a white or black shirt?'') and mathematical reasoning examples for the belief bias (e.g., ``The price is \$10 per soda. The customer inserted \$20. Conclusion: The customer can buy only 1 soda. Answer: Invalid.'').
By using these format-oriented few-shot examples, we aim to help the model understand the structure of the samples without introducing bias into its behavior.
% Therefore, in order to help the model understand the sample format without biasing it in either direction, we experiment with few-shot prompting without the original samples.
% Instead, we use manually curated examples of choices between arbitrary options for the decoy and certainty effects (e.g., "Which would you prefer, a white or black shirt?") and mathematical reasoning examples for the belief bias (e.g. "The price is \$10 per soda. The customer inserted 20\$. Conclusion: The customer can buy only 1 soda. Answer: Invalid.").
% We call this approach \textit{format few-shot} as the intention is to show the model the sample format using few-shot examples.

In the case of the belief bias, there are correct labels.
Therefore we can prompt the model with few-shot samples and avoid biasing the model.
We do that by utilizing samples comprised of neutral non-real objects derived from a distinct set of fabricated words that were deliberately excluded from the test data.
This particular variation is referred to as ``Task few-shot'' since the few-shot samples belong to the same task as the test samples.
By comparing the impact of using few-shot examples solely for formatting purposes (format few-shot) with those pertaining to the same task (Task few-shot) on bias scores, we can evaluate their respective effects.

% the zero-shot setting aligns most effectively with our objective of assessing the model's bias with minimal external influence.

% \textbf{Format Few-Shot}
% \gabis{WDYM by ``Format Few-Shot" -- is this an header? it should still be grammatical}
% In addition to zero-shot, we conducted experiments involving few-shot samples that were intended that presented the model with choices between arbitrary options for the decoy and certainty effects (e.g., "Which would you prefer, a white or black shirt?") with random answers that are constrained to be balanced within the same example (if we have 3-shot examples, we won't have 'Option 1' more than two times).
% This experimental design aimed to explore the impact of exposing the model to the choice format on its subsequent choice patterns.

% For the belief bias, we employed mathematical reasoning examples as few-shot such as "The price is \$10 per soda. The customer inserted 20\$. Conclusion: The customer can buy only 1 soda. Answer: Invalid.".

% \textbf{Task Few-Shot} 
% \gabis{Again, wdym by ``Task Few-Shot''}
% For the belief bias experiments, we can utilize samples comprising non-real objects derived from a distinct set of fabricated words that were deliberately excluded from the test data.
% This approach enables us to assess the impact of using few-shot examples solely for formatting purposes compared to employing few-shot examples pertaining to the same task on the bias scores.





==> Sections/Figures/00_figure1.tex <==
\begin{figure}[t!]
\centering
\begin{minipage}[t]{0.99\columnwidth}
\includegraphics[width=1.0\columnwidth]{Sections/Figures/figure_1_illustrate.pdf}
\caption{Example tasks from \emph{certainty effect} dataset, for the control condition (left) and \biaseddataset{} condition (right), along with typical answers from humans and instruction-tuned models, both of which are biased.
%\nir{the upper line in the image ('In both..') -- could readers think this is part of the task input?} \itay{ran a blind test with a few people - seems to work fine :)}
} 
\label{fig:figure1_example_data}
\end{minipage}
%\qquad\qquad
\qquad
\begin{minipage}[t]{0.99\columnwidth}
\includegraphics[width=0.9\columnwidth]{Sections/Figures/figure_1.pdf}
\caption{%\gabis{Is there actually a blue bar here? It's way too small to notice.} \itay{yes, it's just really small (<0.01). It's a good example for bias which the pretrained model show no bias.}
Bias scores of different GPT3 and GPT3.5 models on the certainty effect dataset.
Similar to human choice behavior,
instruction-tuned models (DaVinci-002 and DaVinci-003) tend to prefer certain outcomes over alternatives that yield higher expected rewards but have some level of risk.
% These models favor the option with a higher expected value unless the alternative option offers the prize with certainty.
In contrast, the pretrained model ('DaVinci') shows no such bias. %Example of \biaseddataset{} and control samples from the certainty effect data (upper).
} 
\label{fig:figure1_example}
\end{minipage}
\end{figure}


==> Sections/Figures/01_examples.tex <==

% \begin{figure*}[t!]
%     \centering
%   \includegraphics[width=1.0\textwidth]{Sections/Figures/examples.pdf}
%     \caption{Examples of the three biases we evaluate: (A) A choice between two prize options, (B) a choice between products with different prices and quality measurements, and (C) assessing the validity of logical syllogisms. In the certainty effect and in the decoy effect, the model must choose the option it prefers, while in the belief bias, the decides if the conclusion is valid or invalid.}
%     \label{fig:biases}
% \end{figure*}


==> Sections/Figures/07_decoy_bias_type_flan.tex <==
\begin{figure}[t!]

\centering
\includegraphics[width=1\columnwidth]{Sections/Figures/decoy_bias_type_flan.pdf}

% \qquad\qquad
\caption{The Impact of Decoy Sub-types on Decoy Cheaper Bias Score for Real-Estate Products in Flan-T5-XXL. Sub-types include \textit{F} (same price, worse quality), \textit{R} and \textit{R*} (higher price, same quality), and \textit{RF} (higher price, worse quality). In contrast to humans, the Flan-T5 model shows higher bias with \textit{F} sub-type compared to \textit{R} and \textit{R*}.}
\label{fig:decoy_type_flan}

\end{figure}


==> Sections/Figures/08_certainty_bias_type.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=1\columnwidth]{Sections/Figures/certainty_bias_type.pdf}
% \qquad\qquad
\caption{The Effect of the Certainty sub-types on the bias score. X axis is the different Certainty sub-type.}
\label{fig:certainty_bias_type}
\end{figure}


==> Sections/Figures/09_certainty_prize.tex <==
% \begin{figure}[t!]
% \centering
% \includegraphics[width=1\columnwidth]{Sections/Figures/certainty_prize.pdf}
% % \qquad\qquad
% \caption{The Effect of the Certainty different prize money in the target option on the bias score. X axis is the prize in dollars.}
% \label{fig:certainty_prize}
% \end{figure}
\begin{figure}[t!]
\centering
\begin{subfigure}[th!]{0.5\textwidth}
\centering
    \includegraphics[width=1\linewidth]{Sections/Figures/certainty_prize_davinci003.pdf}
    \caption{DaVinci-003}
    \label{fig:certainty_prize_davinci003}
\end{subfigure}%
\hfill
\begin{subfigure}[th!]{0.5\textwidth}
\centering
    \includegraphics[width=1\linewidth]{Sections/Figures/certainty_prize_flan.pdf}
    \caption{Flan-T5-XXL}
    \label{fig:certainty_prize_flan}
\end{subfigure}
\caption{The certainty effect bias scores impacted by different prize money in the target option. X axis is the prize in dollars.}
\label{fig:certainty_prize}
\end{figure}

==> Sections/Figures/10_price_range_flan_xxl.tex <==
\begin{figure}[th!]
\centering
\includegraphics[width=1\columnwidth]{Sections/Figures/price_range_flan_xxl.pdf}
% \qquad\qquad
\caption{The Effect of price range on the bias score of the decoy cheaper bias with real-estate products in the Flan-T5-XXL model. The x-axis represents the target price, where an increase in the target price leads to a wider gap between the target and competitor prices. The bias score demonstrates a positive correlation with the increasing price gap, except for the \$100K price where the model chose the competitor 100\% of the time.}
\label{fig:decoy_prices_flan}
\end{figure}


==> Sections/Figures/11_decoy_type_davinci.tex <==
\begin{figure}[th!] 
\centering
\includegraphics[width=1\columnwidth]{Sections/Figures/decoy_bias_type_davinci003.pdf}
\caption{The Impact of Decoy Sub-types on Decoy Cheaper Bias Score for Real-Estate Products in DaVinci-003. Sub-types include \textit{F} (same price, worse quality), \textit{R} and \textit{R*} (higher price, same quality), and \textit{RF} (higher price, worse quality). In contrast to humans, the DaVinci-003 model does not show a strong shift in bias score for different decoy sub-types.}
\label{fig:decoy_type_davinci003}
\end{figure}



==> Sections/Figures/12_certainty_utility_gap.tex <==
\begin{figure}[t!]
\centering
\begin{subfigure}[th!]{0.5\textwidth}
\centering
    \includegraphics[width=1\linewidth]{Sections/Figures/certainty_utility_gap_davinci003.pdf}
    \caption{DaVinci-003}
    \label{fig:certainty_utility_davinci003}
\end{subfigure}%
\hfill
\begin{subfigure}[th!]{0.5\textwidth}
\centering
    \includegraphics[width=1\linewidth]{Sections/Figures/certainty_utility_gap_flan.pdf}
    \caption{Flan-T5-XXL}
    \label{fig:certainty_utility_flan}
\end{subfigure}
\caption{The certainty effect bias scores are impacted by a utility gap between the higher expected value option to the target option. The x-axis is the utility gap.}
\label{fig:certainty_utility_gap}
\end{figure}

==> Sections/Figures/13_pretrained_few_shot.tex <==
\begin{figure}[t!]
\centering
\begin{subfigure}[t]{0.5\textwidth}
\centering
    \includegraphics[width=1\linewidth]{Sections/Figures/format_few_shot_davinci.pdf}
    \caption{DaVinci}
    \label{fig:few_shot_davinci}
\end{subfigure}%
\hfill
\begin{subfigure}[t]{0.5\textwidth}
\centering
    \includegraphics[width=1\linewidth]{Sections/Figures/format_few_shot_t5.pdf}
    \caption{T5-XXL}
    \label{fig:few_shot_T5}
\end{subfigure}
\caption{The impact of format few-shots on bias scores in pretrained LLMs. The utilization of few-shot examples does not results in a significant change in bias scores.}
\label{fig:few_shot_pretrained}
\end{figure}

==> Sections/Figures/15_belief_acc_bias_t5.tex <==
\begin{figure}[t!] 
\centering
\includegraphics[width=1\columnwidth]{Sections/Figures/belief_acc_bias_t5.pdf}
% \qquad\qquad
\caption{The relationship between bias scores and model accuracy on the belief bias task's logical reasoning aspect for the T5-XXL and Flan-T5-XXL models. Similarly to the GPT models, an increase in model accuracy is accompanied by higher bias scores.}
\label{fig:belief_acc_bias_t5}
\end{figure}



==> Sections/Figures/figure_decoy_exm.tex <==
\begin{figure*}[th!]
\centering
\includegraphics[width=1.0\columnwidth]{Sections/Figures/decoy_effect_exm.pdf}
% \qquad\qquad
\caption{Just an example for an illustration.}
\label{fig:decoy_example}
\end{figure*}

==> Sections/Tables/diff_of_diffs.tex <==

% \begin{table*}[th!]
% \centering
% % \small
% \begin{tabular}{@{}llccc  cc@{}}
% \toprule
%  &  & \multicolumn{3}{c}{\textbf{GPT3}} & \multicolumn{2}{c}{\textbf{T5}}  \\
%  \cmidrule(lr){3-5} \cmidrule(lr){6-7}
% & & \textbf{LM} &  \multicolumn{2}{c}{\textbf{Instruction-LM}} & \textbf{LM} & \textbf{Instruction-LM}  \\
% \cmidrule(lr){4-5}
% & \hspace{0.8cm} \textbf{Bias} & DaVinci & DaVinci-002 & DaVinci-003 & T5 & Flan--T5  \\
% \midrule
% \multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{Bias Score}}} 
% & Decoy Expensive & -- 0.15* & -- 0.13* & \textbf{-- 0.02} & \textbf{0.02} & -- 0.18*   \\
% & Decoy Cheaper & --0.17* & -- 0.08* & \textbf{0.08}** & -- 0.15* & \textbf{0.20}*   \\
% %& Certainty & 0.00 & 0.21* & \textbf{0.54}* & 0.09* & \textbf{0.16}*  \\ % this is 3 sub-types
% & Certainty & 0.00 & 0.24* & \textbf{0.67}* & 0.09* & \textbf{0.17}*  \\ % this is two main sub-types
% & Belief Valid & -0.03 & 0.18* & \textbf{0.23}* & 0.00 &\textbf{0.40}*    \\
% % \midrule
% & Belief Invalid & 0.09* & 0.55* & \textbf{0.61}* & 0.01 & \textbf{0.39}*    \\
% \bottomrule
% \end{tabular}
% \caption{The difference between the choices of models in the target option in the \biaseddataset condition versus control conditions. A higher score means the model exhibits a higher level of bias. Results marked with * are statistically significant with p-values $<.05$,  and results marked with ** are  averaged across multiple products where some are significant and others are not.}
% \label{tab:results}
% \end{table*}

==> Sections/Tables/gpt4_results_0_shot.tex <==


\begin{table}[th]
\centering
\begin{tabular}{@{}lc|cc}
\toprule
 & \multirow{2}{*}{\textbf{Bias}}  & \multicolumn{2}{c}{\textbf{Zero-Shot}} \\
& & \textbf{DaVinci-003} & \textbf{GPT4} \\
\midrule
\multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{Bias Score}}} 
& Decoy Expensive &  -- 0.14 & \textbf{0.42}*   \\
& Decoy Cheaper &  0.16 & \textbf{0.20}*   \\
%& Certainty & \textbf{0.54}* & 0.17*   \\ % all three bias types
& Certainty & \textbf{0.67}* & 0.23*   \\ % two bias types
& Belief Valid & \textbf{0.23}* & 0.07*   \\
& Belief Invalid &  \textbf{0.61}* & 0.49*  \\
\bottomrule
\end{tabular}
\caption{comparison of the results between GPT4 and the most recent GPT3.5 release DaVinci-003 in zero-shot setting and zero-shot format. The decoy results are only on one product type (real-estate properties). Scores marked with * are statistically significant with p-values $<.05$}
\label{tab:gpt4_zero-shot_results}
\end{table}

% 0 and 1 shot at once!
%
% \begin{table*}[th]
% \centering
% \begin{tabular}{@{}lccc|cc}
% \toprule
%  & \multirow{2}{*}{\textbf{Bias}} & \multicolumn{2}{c}{\textbf{0-Shot}} & \multicolumn{2}{c}{\textbf{1-Shot}} \\
% & & \textbf{Text-DaVinci-003} & \textbf{GPT4} & \textbf{Text-DaVinci-003} & \textbf{GPT4} \\
% \midrule
% \multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{Bias Score}}} 
% & Decoy Expensive &  -- 0.14 & \textbf{0.42}* & NA & 0.38*  \\
% & Decoy Cheaper &  0.16 & \textbf{0.20}*  & NA  & 0.05  \\
% & Certainty & \textbf{0.54}* & 0.17*  & 0.35  & 0.15*  \\
% & Belief Valid & \textbf{0.23}* & 0.07*  & 0.21 & 0.06*  \\
% & Belief Invalid &  \textbf{0.61}* & 0.49*  & 0.51  & 0.28*  \\
% \bottomrule
% \end{tabular}
% \caption{comparison of the results between GPT4 and the most recent GPT3.5 release 'Text-DaVinci-003' in zero-shot setting and 1-shot format. Scores marked with * are statistically significant with p-values $<.05$}
% \label{tab:gpt4_results}
% \end{table*}



==> Sections/Tables/table_not_probable.tex <==

\begin{table*}[th!]
\centering
% \small
\begin{tabular}{@{}llccc  cc@{}}
\toprule
 &  & \multicolumn{3}{c}{\textbf{GPT3}} & \multicolumn{2}{c}{\textbf{T5}}  \\
 \cmidrule(lr){3-5} \cmidrule(lr){6-7}
& & \textbf{LM} &  \multicolumn{2}{c}{\textbf{Instruction-LM}} & \textbf{LM} & \textbf{Instruction-LM}  \\
\cmidrule(lr){4-5}
& \hspace{0.8cm} \textbf{Bias} & DaVinci & DaVinci-002 & DaVinci-003 & T5 & Flan--T5  \\
\midrule
\multirow{2}{*}{\rotatebox[origin=c]{90}{\textbf{}}} 
%& Certainty & 0.00 & 0.21* & \textbf{0.54}* & 0.09* & \textbf{0.16}*  \\ % this is 3 sub-types
%& Certainty & 0.00 & 0.24* & \textbf{0.67}* & 0.09* & \textbf{0.17}*  \\ % this is two main sub types
& Not Probable & 0.00 & 0.13* & \textbf{0.22}* & 0.08 & \textbf{0.14}*  \\ % this is not probable only
\bottomrule
\end{tabular}
\caption{The difference in bias scores between the choices of models in the target option in the \biaseddataset{} versus control conditions. A higher score means the model exhibits a higher level of bias. Results marked with * are statistically significant with p-values $<.05$.}
\label{tab:not_probable_results}
\end{table*}

==> Sections/Tables/table_options_locations.tex <==

\begin{table*}[th!]
\centering
% \small
\begin{tabular}{@{}llcc|c  cc@{}}
\toprule
 &  & \multicolumn{2}{c}{\textbf{Control}} & \multicolumn{3}{c}{\textbf{\Biaseddataset}}  \\
\cmidrule(lr){3-7}
 \hspace{0.7cm} \textbf{Model} &  \hspace{0.7cm} \textbf{Bias} & Option 1 & Option 2 & Option 1 & Option 2 & Option 3  \\
\midrule
\multirow{3}{*}{ \hspace{0.5cm} DaVinci} 
& Decoy Expensive &                             0.0\% &                           \textbf{100.0\%} &             0.0\% &                        2.2\% &                       \textbf{97.8\%} \\
 &   Decoy Cheaper &                             0.0\% &                           \textbf{100.0\%} &              0.0\% &                        1.5\% &                      \textbf{ 98.5\%} \\
 &       Certainty &            \textbf{ 100.0\%} &                         0.0\% &                     \textbf{ 100.0\%} &                        0.0\% &                       --- \\
 % &    Belief Valid &          74.0\% &                        26.0\% &                       74.0\% &                       26.0\% &                        0.0\% \\
 % &  Belief Invalid &      74.0\% &                        26.0\% &                       74.0\% &                       26.0\% &                        0.0\% \\
\midrule

\multirow{3}{*}{ \hspace{0.1cm} DaVinci-002} 
 & Decoy Expensive &                            71.5\% &                            28.5\% &          45.0\% &                       33.0\% &                       22.2\% \\
 &   Decoy Cheaper &                            75.5\% &                            24.5\% &             36.5\% &                       33.2\% &                       30.2\% \\
 &       Certainty &                    \textbf{ 87.0\%} &                        13.0\% &                       64.0\% &                       36.0\% &                       --- \\
 % &    Belief Valid &                     60.0\% &                        40.0\% &                       45.0\% &                       55.0\% &                        0.0\% \\
 % &  Belief Invalid &                      60.0\% &                        40.0\% &                       45.0\% &                       55.0\% &                        0.0\% \\
\midrule

\multirow{3}{*}{ \hspace{0.1cm} DaVinci-003} 
 & Decoy Expensive &                            77.0\% &                            23.0\% &      48.5\% &                       32.5\% &                       18.8\% \\
 &   Decoy Cheaper &                            79.0\% &                            21.0\% &      50.3\% &                       26.8\% &                       23.0\% \\
 &       Certainty &          57.0\% &                        43.0\% &                       44.0\% &                       56.0\% &                       --- \\
 % &    Belief Valid &      43.0\% &                        57.0\% &                       35.0\% &                       65.0\% &                        0.0\% \\
 % &  Belief Invalid &              43.0\% &                        57.0\% &                       35.0\% &                       65.0\% &                        0.0\% \\

\midrule

\multirow{3}{*}{ \hspace{0.7cm} GPT4} 
 & Decoy Expensive &                            63.0\% &                            37.0\% &           38.2\% &                       27.5\% &                       33.5\% \\
  &   Decoy Cheaper &                            78.0\% &                            22.0\% &          44.2\% &                       23.0\% &                       32.8\% \\
  &       Certainty &                    52.0\% &                        48.0\% &                       47.0\% &                       53.0\% &                        --- \\
  % &    Belief Valid &                     34.0\% &                        62.0\% &                       35.0\% &                       65.0\% &                        0.0\% \\
  % &  Belief Invalid &                     34.0\% &                        62.0\% &                       35.0\% &                       65.0\% &                        0.0\% \\
\midrule

\multirow{3}{*}{ \hspace{0.5cm} T5-XXL} 
 & Decoy Expensive &                            12.8\% &                            \textbf{87.2\%} &       33.5\% &                       47.0\% &                       20.0\% \\
 &   Decoy Cheaper &                            12.8\% &                           \textbf{ 87.2\%} &            33.2\% &                       48.8\% &                       18.0\% \\
 &       Certainty &                    31.0\% &                        69.0\% &                       32.0\% &                       68.0\% &                       --- \\
% &    Belief Valid &                      7.0\% &                        \textbf{93.0\% }&                        5.0\% &                       \textbf{95.0\%} &                        0.0\% \\
%  &  Belief Invalid &                       7.0\% &                        \textbf{93.0\%} &                        5.0\% &                      \textbf{ 95.0\%} &                        0.0\% \\

\midrule

\multirow{3}{*}{ \hspace{0.1cm} Flan-T5-XXL} 
 & Decoy Expensive &                            49.2\% &                            50.8\% &        45.2\% &                       35.0\% &                       20.0\% \\
 &   Decoy Cheaper &                            49.5\% &                            50.5\% &         44.0\% &                       25.8\% &                       30.0\% \\
 &       Certainty &                   44.0\% &                        56.0\% &                       38.0\% &                       62.0\% &                       --- \\
 % &    Belief Valid &                    32.0\% &                        68.0\% &                       28.0\% &                       65.0\% &                        0.0\% \\
 % &  Belief Invalid &               32.0\% &                        68.0\% &                       28.0\% &                       65.0\% &                        0.0\% \\
\bottomrule

\bottomrule
\end{tabular}
\caption{ Percentage of option location preferences across all samples for each model and bias.
The results reveal consistent patterns in the choice behavior of pretrained models, where DaVinci exhibits an absolute preference for a specific location in 100\% of the cases in the decoy and certainty effects. Similarly, T5-XXL shows a preference in over 87\% of the cases in the control decoy effects. In contrast, the remaining models exhibit varying tendencies towards specific option locations that are contingent upon the content of the options. Notably, DaVinci-002 demonstrates an 87\% preference for option 1 in the certainty effect.}
\label{tab:options_locations}
\end{table*}

==> Sections/Tables/table_products.tex <==
\begin{table*}[th!]
\centering
% \small
\begin{tabular}{@{}llccc  cc@{}}
\toprule
 &  & \multicolumn{3}{c}{\textbf{GPT3}} & \multicolumn{2}{c}{\textbf{T5}}  \\
 \cmidrule(lr){3-5} \cmidrule(lr){6-7}
& & \textbf{LM} &  \multicolumn{2}{c}{\textbf{Instruction-LM}} & \textbf{LM} & \textbf{Instruction-LM}  \\
\cmidrule(lr){4-5}
\hspace{1.2cm} \textbf{Bias} & \hspace{0.3cm} \textbf{Product} & DaVinci & DaVinci-002 & DaVinci-003 & T5 & Flan--T5  \\
\midrule

\multirow{4}{*}{{\hspace{0.3cm} \textbf{Decoy Expensive}}} 
& Frying Pan & -- 0.12*  &  \hspace{0.1cm}  -- 0.23* & \textbf{-- 0.06} &  \hspace{0.15cm} \textbf{0.14}* &  -- 0.19*  \\
& Phone & -- 0.16* & -- 0.08 &  \hspace{0.1cm} \textbf{0.03} &  \hspace{0.15cm} \textbf{0.10}* & -- 0.09*   \\
& Car & -- 0.16* & -- 0.07  & \hspace{0.2cm} \textbf{0.09}* & -- \textbf{0.15}* &  -- 0.24*  \\
& Real-Estate & -- 0.17* & -- \textbf{0.13}*  &  \hspace{0.05cm} -- 0.14* & -- \textbf{0.01}  &  -- 0.19*  \\

\midrule

\multirow{4}{*}{{\hspace{0.2cm} \textbf{Decoy Cheaper}}} 
& Frying Pan & -- 0.18* &  \hspace{0.1cm} 0.03 &  \hspace{0.1cm} \textbf{0.11}* &  \hspace{0.1cm} -- 0.06 &  \textbf{0.22}*  \\
& Phone & -- 0.17* & -- 0.10* & \textbf{0.01}  & -- 0.10* &  \textbf{0.35}*  \\
& Car & -- 0.17* & -- 0.12*  & \textbf{0.04}  & -- 0.15*  &  \textbf{0.16}*  \\
& Real-Estate & -- 0.17* & -- 0.14* &  \hspace{0.1cm} \textbf{0.16}* &  -- 0.27* & \textbf{0.08}*   \\



\bottomrule
\end{tabular}
\caption{The bias scores for different products in the decoy expensive and decoy cheaper effects. A higher score means the model exhibits a higher level of bias. Results marked with * are statistically significant with p-values $<.05$.}
\label{appendix:tab:products_results}
\end{table*}
